EAGLE: Enhanced Visual Grounding Minimizes Hallucinations in Instructional Multimodal Models

Large language models and vision transformers have demonstrated impressive zero-shot capabilities, enabling significant transferability in downstream tasks. The fusion of these models has resulted in multi-modal architectures with enhanced instructional capabilities. Despite incorporating vast image and language pre-training, these multi-modal architectures often generate responses that deviate from the ground truth in the image data. These failure cases are known as hallucinations. Current methods for mitigating hallucinations generally focus on regularizing the language component, improving the fusion module, or ensembling multiple visual encoders to improve visual representation. In this paper, we address the hallucination issue by directly enhancing the capabilities of the visual component. Our approach, named EAGLE, is fully agnostic to the LLM or fusion module and works as a post-pretraining approach that improves the grounding and language alignment of the visual encoder. We show that a straightforward reformulation of the original contrastive pre-training task results in an improved visual encoder that can be incorporated into the instructional multi-modal architecture without additional instructional training. As a result, EAGLE achieves a significant reduction in hallucinations across multiple challenging benchmarks and tasks.

==> figures/qualitative_exams.tex <==
\begin{figure*}[t]
    \centering
    % First subfigure (a)
    \begin{subfigure}[b]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/qua_exam_1.png}
        \caption{}
        \label{fig:figure1}
    \end{subfigure}

    
    % Second subfigure (b)
    \begin{subfigure}[b]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/qua_exam_2.png}
        \caption{}
        \label{fig:figure2}
    \end{subfigure}
    
    \caption{Overall caption for both figures (a) and (b).}
    \label{fig:qualitative_exam}
\end{figure*}

==> figures/teaser_fig_old.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/teaser_fig.png}
    \caption{\textbf{\methodname visual encoders reduce hallucinations in IT-VLM.} We present three example scenarios, each featuring a question about an image posed to a specific IT-VLM with its original visual encoder (left pink box) and the corresponding EAGLE-tuned visual encoder (right orange box). “IB7", “IB13" and “IBT5" refer to InstructBLIP with Vicuna7B, Vicuna13B, and FlanT5xl, respectively. EAGLE substantially reduces hallucinations, providing more visually grounded and reliable descriptions. \textbf{i)} In the first example (left), IB13 with the EAGLE-tuned visual encoder can clearly identify fine-grained elements such as a fence, house, and trees. \textbf{ii)} In the second example (center), EAGLE helps IB7 to accurately recognize a dog, even in an unusual viewpoint and context. \textbf{iii)} In the third example (right), EAGLE enhances object localization, allowing the model to precisely identify the laptop’s position. These examples illustrate EAGLE’s effectiveness in improving visual grounding across complex, multi-object scenes.}
    \label{fig:teaser_fig}
\end{figure*}


==> tables/itlvlm_benchmark.tex <==
\begin{table*}[t]
    
    \centering
     \caption{
        \textbf{Results for Inter-object Relationship Understanding.} 
    }
    
    \resizebox{18cm}{!}{
    \begin{tabular}{l l l rrrr |r|rrrrr} % creating eight columns
        \toprule
        
        \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} &  \multicolumn{1}{c}{\multirow{2}{*}{\bf Visual Encoder}} & \multicolumn{1}{c}{\multirow{2}{*}{\bf LLM}} & \multicolumn{4}{c}{\bf POPE} & \multicolumn{1}{c}{\bf MMVP} & \multicolumn{5}{c}{\bf MERLIM}
        \\\cmidrule(lr){4-13}
             & & & \multicolumn{1}{c}{$ \bf Acc \uparrow$} & \multicolumn{1}{c}{$ \bf F1 \uparrow$} & \multicolumn{1}{c}{$\bf Prec \uparrow $} & \multicolumn{1}{c}{$\bf Rec \uparrow$} & \multicolumn{1}{c}{$\bf Acc \uparrow$} & \multicolumn{1}{c}{$\bf Prec^{1}_{Orig} \uparrow$} & \multicolumn{1}{c}{$\bf Prec^{1}_{Inp} \uparrow$} & \multicolumn{1}{c}{$\bf Prec^{2}_{Orig} \uparrow$} & \multicolumn{1}{c}{$\bf Prec^{2}_{Inp} \uparrow$}
             \\
        \midrule
        BLIP-2 & EVA01 ViT-g-14 & FlanT5xl & 69.33\% & 70.90\% & 67.34\% & 75.06\% & 14.0\% & 57.68\% & 47.06\% & 58.93\% & 48.48\%
        \\
        \rowcolor{LightCyan}
        BLIP-2 & Eagle EVA01 ViT-g-14 & FlanT5xl & \bf 71.40\% & \bf 72.81\% & \bf 69.40\% & \bf 76.60\% & \bf 15.33\% & \bf 59.39\% & \bf 48.64\% & \bf 62.35\% & \bf 50.37\%
        \\
        \cmidrule{1-13}
        InstructBLIP & EVA01 ViT-g-14 & Vicuna-7B v1.1 & 75.0\% & 77.99\% & 69.73\% & \bf 88.47\% & 18.0\% & 56.38\% & 49.02\% & 43.45\% & 39.89\%
        \\
        \rowcolor{LightCyan}
        InstructBLIP & Eagle EVA01 ViT-g-14 & Vicuna-7B v1.1 & \bf 77.20\% & \bf 79.39\% & \bf 72.44\% & 87.80\% & \bf 20.67\% & \bf 59.11\% & \bf 50.97\% & \bf 46.14\% & \bf 41.41\%
        \\
        %\cmidrule{1-11}
        InstructBLIP & EVA01 ViT-g-14 & Vicuna-13B v1.1 & 64.43\% & 73.73\% & 59.46\% & \bf 97.0\% & \bf 24.67\% & 36.58\% & 32.32\% & 32.08\% & 28.28\%
        \\
        \rowcolor{LightCyan}
        InstructBLIP & Eagle EVA01 ViT-g-14 & Vicuna-13B v1.1 & \bf 67.57\% & \bf 74.92\% & \bf 61.08\% & 96.8\% & \bf 24.67\% & \bf 40.60\% & \bf 35.50\% & \bf 34.96\% & \bf 31.01\%
        \\
        %\cmidrule{1-11}
        InstructBLIP & EVA01 ViT-g-14 & FlanT5xl & 58.0\% & 70.0\% & 54.44\% & \bf 98.0\% & 18.0\% & 41.40\% & 38.19\% & 44.48\% & 39.78\%
        \\
        \rowcolor{LightCyan}
        InstructBLIP & Eagle EVA01 ViT-g-14 & FlanT5xl & \bf 59.83\% & \bf 70.92\% & \bf 55.58\% & 97.93 & \bf 19.33\% & \bf 43.47\% & \bf 38.64\% & \bf 47.95\% & \bf 42.91\% 
        \\
        \cmidrule{1-13}
        LLaVA-1.5 & OpenAI ViT-L-14-336 & Vicuna-7B v1.5 &  69.33\% & 76.10\% &  62.34\% & 97.67\% & 25.33\% & 49.14\% & 43.10\% & 30.47\% & 28.93\%
        \\
         \rowcolor{LightCyan}
         LLaVA-1.5 & Eagle OpenAI ViT-L-14-336 & Vicuna-7B v1.5 & 67.53\% & 74.93\% & 61.02\% & 97.07\% & \textbf{26.66\%} & \bf 50.47\% & \bf 43.45\% & 30.41\% & 28.39\%
        \\
        \rowcolor{LightCyan}
        LLaVA-1.5* & Eagle OpenAI ViT-L-14-336 & Vicuna-7B v1.5 & -- & -- & -- & -- & -- & 48.47\% & 43.24\% & \bf 37.85\% & \bf 33.06\%
        \\
        \bottomrule
    \end{tabular}
}
   
    \label{tab:itlvlm_results}
    \vspace{-0.825em}
\end{table*}

==> tables/vlm_benchmark_ZS.tex <==
\begin{table*}
    
    \caption{
        \textbf{ZST RESULTS.} 
    }\vspace{-0.2cm}
    
    \resizebox{17cm}{!}{
        \begin{tabular}{l ll | llll} % creating eight columns
            \toprule
            
            \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} &  \multicolumn{2}{c}{\bf IN-1K Zero-Shot} & \multicolumn{4}{c}{\bf MSCOCO Hallucination}
            \\\cmidrule(lr){2-7}
                 & \multicolumn{1}{c}{\bf Cls Acc $\uparrow$} & \multicolumn{1}{c}{ \bf Seq. Acc $\uparrow$} & \multicolumn{1}{c}{\bf Seq. Hall@1 $\downarrow$} & \multicolumn{1}{c}{\bf Seq. Hall@3 $\downarrow$} & \multicolumn{1}{c}{\bf Seq. Hall@5 $\downarrow$} & \multicolumn{1}{c}{\bf Seq. Hall@10 $\downarrow$}
                 \\
            \midrule
            EVA01 ViT-g-14 & \bf 78.50\% & 57.76\% & 24.64\% & 56.68\% & 68.17\% & 79.77\%  
            \\
            \rowcolor{LightCyan}
            Eagle EVA01 ViT-g-14 & 76.65\% \footnotesize\textcolor{red}{(-1.85\%)} & \bf 65.81\% \footnotesize\textcolor{ForestGreen}{(+8.05\%)} & \bf 5.11\% \footnotesize\textcolor{ForestGreen}{(-19.53\%)} & \bf 39.57\% \footnotesize\textcolor{ForestGreen}{(-17.11\%)} & \bf 57.77\% \footnotesize\textcolor{ForestGreen}{(-10.4\%)} & \bf 75.62\% \footnotesize\textcolor{ForestGreen}{(-4.15\%)} 
            \\
            \cmidrule{1-7}
            OpenAI ViT-L-14-336 & \bf 76.55\% & 0.7\% & 43.74\% & 67.63\% & 77.09\% & 86.0\%
            \\
             \rowcolor{LightCyan}
             Eagle OpenAI ViT-L-14-336 & 71.46\% \footnotesize\textcolor{red}{(-5.09\%)} & \bf 50.98\% \footnotesize\textcolor{ForestGreen}{(+50.28\%)} & \bf 29.54\% \footnotesize\textcolor{ForestGreen}{(-14.2\%)} & \bf 51.35\% \footnotesize\textcolor{ForestGreen}{(-16.28\%)} & \bf 63.64\% \footnotesize\textcolor{ForestGreen}{(-13.45\%)} & \bf 77.63\% \footnotesize\textcolor{ForestGreen}{(-8.37\%)}
            \\
            \bottomrule
        
        \end{tabular}
    }
   
    \label{tab:zst_results}
\end{table*}


